Unraveling BitTorrent's File Unavailability: Measurements, Analysis and Solution Exploration

BitTorrent suffers from one fundamental problem: the long-term availability of content. This occurs on a massive-scale with 38% of torrents becoming unavailable within the first month. In this paper we explore this problem by performing two large-scale measurement studies including 46K torrents and 29M users. The studies go significantly beyond any previous work by combining per-node, per-torrent and system-wide observations to ascertain the causes, characteristics and repercussions of file unavailability. The study confirms the conclusion from previous works that seeders have a significant impact on both performance and availability. However, we also present some crucial new findings: (i) the presence of seeders is not the sole factor involved in file availability, (ii) 23.5% of nodes that operate in seedless torrents can finish their downloads, and (iii) BitTorrent availability is discontinuous, operating in cycles of temporary unavailability. Due to our new findings, we consider it is important to revisit the solution space; to this end, we perform large-scale trace-based simulations to explore the potential of two abstract approaches.

==> conclusions.tex <==
\section{Conclusions}
This paper has investigated BitTorrent's unavailability problem in the wild and explored the feasibility of the potential solution-space. To achieve this, two large-scale measurements studies were performed to ascertain the characteristics, causes and repercussions of file unavailability in BitTorrent. Based on this, we made a number of interesting findings that offer the most accurate study of file availability in BitTorrent so far. Most notably, it was found that $(i)$ a lack of seeders often results in unavailability but \textit{not} always, $(ii)$ the churn level, the fast replication of rare chunks and the population size largely defines a swarm's ability to survive without a seeder $(iii)$ unavailability usually occurs in cyclic periods with intermittent availability, and $(iv)$ unavailability often results in a chain effect that leads to future download failures.

Due to these new findings, the solution-space was also investigated to see how they affect both single and cross torrent solutions. It was found that the continuance of BitTorrent's single-torrent mechanisms can only address the problem with a 10 fold increase in seeding times. In contrast, great potential has been found in using the cross-torrent approach which maintains current performance levels whilst also achieving over 99\% availability.




%From the above analysis, it becomes evident that the problem of unavailability can be addressed most appropiately by incentivising users to seed in torrents. Using trace-based simulations, we therefore have inspected the potential of two possible approaches, representing the basic archetypes in the solution space for this problem. The first takes the traditional single-torrent approach of trying to get users to remain in an individual torrent for longer periods whilst the second takes a cross-torrent approach of fostering cooperation between users operating in different torrents. We have found that the continuance of BitTorrent's single-torrent mechanisms can only address the problem with a 10 fold increase in seeding times. In contrast, we have found great potential in using the cross-torrent approach which maintains current performance levels whilst also achieving over 99\% availability.   








%In this work we have conducted two-large scale measurement studies to investigate the file availability problem of BitTorrent in the wild. These measurements have been used to characterise the nature, scale, causes and repercussions of unavailability. Through this analysis, we then designed and simulated a novel cross-torrent solution based on indirect reciprocation. We can therefore now make the following conclusions
%\begin{itemize}
% \item \textit{Nature:} Unavailability is not immutable with intermittent periods of availability lasting a median of 2.36 hours.
% \item \textit{Scale:} Unavailability is a large-scale problem affecting over 38\% of torrent within their first month. This directly affected 1.59 million users from our study.
% \item \textit{Cause:} Seeders are the primary cause of unavailability with 88\% of seedless torrents being unavailable. This arises because seeding times and too short to result in the generation of new (replacement) seeders in the long-term.
% \item \textit{Solution:} Intuitive single-torrent and cross-torrent solutions are largely ineffecive. Instead, a cross-torrent solution based on indirect reciprocation achieves a sucess rate of ~99\%
%\end{itemize}


%Based on these measurements, we have first characterised the nature of file unavailability in BitTorrent while highlighting the problem's seriousness. It has been demonstrated that the file unavailability problem primarily occurs because currently the seeding times are not sufficiently long to support the generation of new (replacement) seeders. This is exacerbated by long user inter-arrival times that reduce the chances of leechers completing their download. Accordingly, the combination of these two factors induce seedless states in which leechers are often not capable of reconstructing a file. Because of the discontinuous seeding behavior of the users, however, content availability is typically discontinuous with intermittent availability. To overcome this problem, we have explored the possible solution space and proposed a feasible cross-torrent solution with we have evaluated through extensive trace-based simulations. Our main findings are:







==> methodology.tex <==

%%%%% OLD. Methodology is now in background.tex



\section{Measurement Methodology}
\label{sec:methodology}
\vspace{-0.3cm}
%In order to investigate file availability in real BitTorrent swarms, it is necessary to connect to the individual nodes and retrieve detailed information such as the node's bitfield. By periodically repeating this process, we can infer insights on the percentage of available chunks (= U(T)) at a given time. In addition, we also infer information about the node's download progress which in turn allows us to compute download rates. As this crawling technique allows us to study the individual behavior of a user under a microscope, we name this \teytit{microscopic crawling}. 

%Obviously, the above approach does not scale very well with increasing number of users, e.g., it is hardly possible to be periodically be connected to millions of users at the same time. Therefore, in order to understand the peer access patterns of the users as well as the dynamics of seeder-to-leecher on a large scale, we have implemented an additional crawler that provides us a high-level view into the system on a per-torrent basis.


%We have conducted two kinds of measurement studies in BitTorrent. The first, the macroscopic measurements,  provides us a high-level view into the system on a per-torrent basis. The second, the microscopic measurements, gives us insight into the individual behaviour of peers.



%%%%
To study the unavailability problem and specifically seeders' role in it, it is important to understand the behaviour of peers in real-world torrents. To achieve this we have performed two large-scale measurement studies: two microscopic studies and a single macroscopic one.


\textbf{\textit{Microscopic Crawling}:} To truly understand unavailability in BitTorrent it is necessary to be able to view the distribution of chunks within any given swarm. Without this, it is only possible to infer availability based on alternative related metrics such as the number of seeders. This is a strong criticism of previous studies that have been prevented from gaining insight into the behaviour of individual peers due to the limitations of only accessing higher-level information \cite{guo:imc}. To gain this information we therefore developed and deployed a BitTorrent crawler that can investigate swarms on a microscopic level. The crawler operated from July 18, 2009 to July 29, 2009 (\textit{micros-1}) and then again from August 19, 2009 to September 5, 2009 (\textit{micros-2}). In order to discover all the online users in a torrent, we rely on two techniques. First, we periodically contact the torrent's tracker that provides us a partial view of the swarm, usually consisting of 50-200 randomly chosen peers. As this view is very limited, we additionally use the Peer Exchange Protocol (PEX) to discover new peers. In a time resolution of 10 minutes, we request for each known peer the chunk bitmap as well its routing table entries (using PEX). To prevent the blacklisting of monitor IP addresses, the request process was distributed over 20 nodes hosted on the Emulab \cite{emulab} testbed. All information was logged creating 7 GB and 12 GB of data in micros-1 and micros-2, respectively. For the \textit{micros-1} study, the crawler followed 255 torrents appearing on Mininova after the first measurement hour. In these torrents, we observed 246,750 users. The \textit{micros-2} dataset contains information from 577 torrents and 531,089 users, respectively. 

\textbf{\textit{Macroscopic Crawling}:} The microscopic measurements provide detailed insight into the distribution of chunks within the swarm as well as between different peers. However, due to scalability issues it is impossible to perform such detailed measurements on a extremely large-scale (e.g. $>$ 1000 torrents). To complement these results we therefore also implemented a crawler that followed every torrents published on the Mininova website in a much higher-level manner after December 09, 2008 for a period of 38 days. This crawler repeatedly requests, from multiple sites in Europe, information regarding each torrent's number of seeders and leechers. By doing so, we were able to continuously discover 98\% of the online peers reported by the tracker. With this information, it is possible to use a similar approach to \cite{biersack:dissecting, guo:journal} to identify different users; we assume a user comes online the first time it is reported by the tracker, and stays online until it is no longer included in the tracker report. This study allowed us to gain an extremely large number of measurements regarding such things as peer arrival patterns, seeder:leecer ratios and torrent sizes. This information can subsequently be correlated with our smaller-scale microscopic measurements to derive such things as the scale of seedless states and the causes for seedless states occuring. Our final macroscopic dataset consisted of reports from 46,227 torrents and 29,066,139 users. 

In the remainder of this paper, we will use both kind of measurements simultaneously for our analysis. 

==> related_work.tex <==
\section{Related Work} \label{sec:relatedwork}

\textbf{BitTorrent Measurements}: 
BitTorrent measurement studies can be classified into two different groups. The first type uses log traces from trackers \cite{biersack:dissecting, guo:journal, guo:imc, trace:umass} whereas the second type relies on crawling techniques to retrieve the information from the system \cite{delft, georgos, ross, towsley, piatek:onehop}. The first type of measurements is less intrusive since they do not actively interfere with the system. However, they are often problematic to obtain since they require the agreement from content providers. The crawling techniques, on the other hand, can be divided into two categories. In its simplest form, a crawler exploits the BitTorrent protocol to periodically request the IP addresses of the clients participating in the torrent from the tracker \cite{ross}. This makes it possible to study the demographics and dynamics of the torrents under analysis. This is what we name \textit{macroscopic crawling}. More sophisticated crawlers also contact the clients and retrieve detailed information such as the client ID and their piece bitmap. We name this \textit{microscopic crawling}. Although the microscopic crawling gives more detailed information, it is noticeably less scalable and only allows a few thousand torrents to be studied in parallel \cite{delft, georgos}. Each approach is effective for addressing particular needs; however, these have not yet been combined to investigate BitTorrent in a holistic way.

%To best of our knowledge, the current paper is the first combining both microscopic and macroscopic crawling techniques to better understand BitTorrent properties, concretely the file availability of BitTorrent.



\textbf{BitTorrent's File Availability Analysis}: 
There are only a few works investigating availability issues in BitTorrent systems \cite{guo:imc, dht-availibility, towsley}. Neglia et al. mainly study the tracker/DHT availability of 22,000 torrents obtained from two torrent indexing sites \cite{dht-availibility}. Guo et al. \cite{guo:imc} extended this, to model the lifespan of torrents by analyzing a limited number of tracker traces from \cite{dht-availibility}; it was found that most torrents are short-lived because of an exponentially decreasing peer arrival rate. 
%This, however, is only based on a small, closed community. 
This model starts from the basis that content is unavailable when there are no seeders present in the swarm. This is, so far, an unverified hypothesis that is important to investigate.
%The model also assumes that once a torrent is devoid of seeders, the torrent is dead and the content unavailable; this assumption has not yet been verified though.
%We have found, however, that both conditions do not uphold in larger communities such as Mininova. 
Similarly, Menasche et al. also use this hypothesis to investigate the availability of seeders in 45,000 torrents obtained from the Mininova website \cite{towsley}, finding that 40\% of swarms lack seeders for more than 15 days in the first month after the torrent's birth. 
%This information is confirmed by our studies, however, we also go significantly further and investigate the causes and real-time repercussions of seedless states as well as the role of seeders and leechers in the process.


\textbf{Improving BitTorrent File Availability}: 
Surprisingly, little research work has been performed into addressing the file availability in BitTorrent \cite{guo:journal, towsley, crosstorrent}. The most recent work improves file availability problem in BitTorrent by file bundling to enlarge the online times of the users. Using a queuing theoretic model and controlled experiments on PlanetLab, the authors show that this approach can reduce waiting-time for peers in torrents with highly unavailable seeders. However, their results consider that peers arrive in a constant Poisson process which is a strong assumption given the measurement results presented in \cite{delft, guo:journal} and also in this paper.

Guo et al. were the first to propose intriguing ideas and results for \textit{cross-torrent collaboration}. Amongst other things, the authors sketch an abstract mechanism for instant inter-torrent collaboration; following this they also evaluate the principles. Yang et al. propose a variation of these ideas by designing a cross-torrent tit-for-tat strategy that assumes repeated interactions of the users. However, this method suffers because as Piatek et al. show through extensive measurements, 91.5\% of peer pairs that occur in a single swarm will never meet again at any later point in time \cite{piatek:onehop}. Piatek et al. subsequently propose an alternative protocol that enables long-term incentives in BitTorrent with the aid of one-hop intermediaries. 

%This paper is orthogonal to all these works as our main intention is to explore file availability in the wild, and objectively investigate the potential of the solution spaces (including single-torrent and cross-torrent approaches). 

%To achieve this, However, we have found that previous investigations have lacked important information regarding file unavailability in BitTorrent. Specifically, they lack the collective data to introspect the behaviour of individual torrents, individual peers and subsequently the system as a whole. This means that existing measurements alongside any evaluative results based have made potentially incorrect assumptions. This paper therefore attempts to address these concerns by offering the first empirical investigation using a large-scale data set into $(i)$ file unavailability in BitTorrent - its causes and effects, and $(ii)$ the potential of the solution space based on this data.

